Causality Analysis for Concurrent Reactive Systems (Extended Abstract)

We present a comprehensive language theoretic causality analysis framework for explaining safety property violations in the setting of concurrent reactive systems. Our framework allows us to uniformly express a number of causality notions studied in the areas of artificial intelligence and formal methods, as well as define new ones that are of potential interest in these areas. Furthermore, our formalization provides means for reasoning about the relationships between individual notions which have mostly been considered independently in prior work; and allows us to judge the appropriateness of the different definitions for various applications in system design. In particular, we consider causality analysis notions for debugging, error resilience, and liability resolution in concurrent reactive systems. Finally, we present automata-based algorithms for computing various causal sets based on our language-theoretic encoding, and derive the algorithmic complexities.

==> eptcsdata.tex <==
\providecommand{\firstpage}{31}
\providecommand{\publicationstatus}{B.~Finkbeiner and S.~Kleinberg: Third International Workshop\\ on Formal Reasoning about Causation, Responsibility,\\ and Explanations in Science and Technology (CREST 2018)\\
EPTCS 286, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.286.3}{10.4204/EPTCS.286.3}}

